AetherVision-Bench: An Open-Vocabulary RGB-Infrared Benchmark for Multi-Angle Segmentation across Aerial and Ground Perspectives

Open-vocabulary semantic segmentation (OVSS) involves assigning labels to each pixel in an image based on textual descriptions, leveraging world models like CLIP. However, they encounter significant challenges in cross-domain generalization, hindering their practical efficacy in real-world applications. Embodied AI systems are transforming autonomous navigation for ground vehicles and drones by enhancing their perception abilities, and in this study, we present AetherVision-Bench, a benchmark for multi-angle segmentation across aerial, and ground perspectives, which facilitates an extensive evaluation of performance across different viewing angles and sensor modalities. We assess state-of-the-art OVSS models on the proposed benchmark and investigate the key factors that impact the performance of zero-shot transfer models. Our work pioneers the creation of a robustness benchmark, offering valuable insights and establishing a foundation for future research.

==> sec/2_relatedworks.tex <==


% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.50]{sec/aaai_table3.png}
%     \caption{D.A improving consistently.}
%     \label{fig:inra}
% \end{figure}



\section{Related works}
\label{sec:formatting}
\begin{table*}[ht]

\centering
\label{table:Dataset comparison}
\begin{adjustbox}{max width=1.0\textwidth}
\begin{tabular}{l c c c c c c c}
\toprule
\textbf{Datasets} & \multicolumn{1}{l}{\textbf{Multi-sensory}} & \multicolumn{1}{l}{\textbf{Diverse Viewpoints}} & \multicolumn{1}{l}{\textbf{Diverse backgrounds}} & \multicolumn{1}{l}{\textbf{Diverse classes}} & \multicolumn{1}{l}{\textbf{Diverse illumination}} & \multicolumn{1}{l}{\textbf{Detection}} & \multicolumn{1}{l}{\textbf{Segmentation}}\\
\midrule
DOTA \cite{xia2018dota}             & \ding{55}                                          & \ding{55}                                                & \ding{55}                                                 & \checkmark                                             & \ding{55}                                    & \checkmark                 & \ding{55}          \\
HIT-UAV \cite{suo2023hit}         & \ding{55}                                           & \checkmark                                                & \checkmark                                                 & \ding{55}                                             & \ding{55}                             & \checkmark                   & \ding{55}               \\
VisDrone \cite{cao2021visdrone}        & \ding{55}                                           & \checkmark                                                & \checkmark                                                 & \checkmark                                             & \checkmark                        & \checkmark                   & \ding{55}                                       \\
UAVDT  \cite{du2018unmanned}           & \ding{55}                                           & \checkmark                                                & \checkmark                                                 & \checkmark                                             & \checkmark                        & \checkmark                   & \ding{55}                                       \\
Vedai \cite{razakarivony2016vehicle}            & \checkmark                                           & \ding{55}                                                & \checkmark                                                 & \checkmark                                             & \checkmark               & \checkmark                   & \ding{55}                                                \\
M3FD \cite{liu2022target}             & \checkmark                                           & \ding{55}                                                & \checkmark                                                 & \checkmark                                             & \checkmark                        & \checkmark                   & \ding{55}                                       \\
FLIR \cite{fliresh}            & \checkmark                                           & \ding{55}                                                & \checkmark                                                 & \checkmark                                             & \checkmark                               & \checkmark                   & \ding{55}                                \\
MSRS \cite{tang2022piafusion}          & \checkmark                                           & \ding{55}                                              & \checkmark                                                 & \checkmark                                             & \checkmark                                & \ding{55}                   & \checkmark                               \\
InfraParis \cite{franchi2024infraparis}  & \checkmark                                           & \ding{55}                                              & \checkmark                                                 & \checkmark                                             & \checkmark                                & \checkmark                   & \checkmark                               \\
{\textbf{IndraEye (Ours)}}   & \checkmark                                           & \checkmark                                                & \checkmark                                                 & \checkmark                                             & \checkmark                                & \checkmark                   & \checkmark                               \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Qualitative comparison of multiple aerial vehicle object detection datasets.}
\label{Qual_comp}
\end{table*}


% Recent advancements in object detection using aerial imagery have been significantly influenced by the availability of diverse datasets captured through Electro-Optical (EO) cameras. These datasets are generally classified based on their viewing angles: (1) nadir or bird’s-eye view datasets, such as VEDAI and DOTA, and (2) oblique or slant-angle datasets, including VisDrone and HIT-UAV. Prominent contributions from datasets like UAVDT and VisDrone have underscored the critical role of UAV-based object detection, driving considerable progress in this domain. These datasets are widely utilized for applications such as aerial perception and traffic monitoring, offering images with diverse viewpoints, backgrounds, and lighting conditions. However, object detection algorithms often face challenges in nighttime settings. While EO cameras deliver high-resolution imagery with detailed textures under adequate lighting, their performance declines in low-light environments due to the lack of sufficient texture details, resulting in reduced detection accuracy.
\textbf{Thermal Object Detection}
% With the technical advances in computing and sensors, the work on RGB object detection has gained significant progress in the fields of robotics, autonomous vehicles for various applications. Similar trends are observed in IR object detection recently. 
% \vspace{-1em}
%%%%%%%%%%%%%%%%CORRECT%%%%%%%%%%%%%%%%%%%%%%%%
% Object detection task using thermal images has been regarded as important area of research in computer vision mainly for military applications such as surveillance, drone reconnaissance, and autonomous driving. Particularly, Aerial Thermal Object Detection (ATOD) faces lot of challenges due to variations in size of the objects and background.  In order to improve the thermal object detection works such as \textbf{cite some gen ai stuff} use GAN to generate IR or RGB images or vice-versa using one of the modality to avoid manual dataset annotation. Several works including \textbf{cite fusion algos} have been proposed to use both modalities by fusing the images when the dataset contains images that are co-registered. Recently few works make use of misaligned RGB-IR images for object detection as seen in \textbf{cite the IEEE transaction and science direct paper}. This clearly shows that the trend of relying on co-registerd dataset is not practically feasible and the need to account for this problem using modern approaches such as Domain adaptation and feature fusion. Several image fusion methods \cite{liu2022target}, \cite{zhao2023cddfuse} have also been proposed to integrate co-registered modalities.
%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Object detection using thermal images has become a critical research area in computer vision, with Aerial Thermal Object Detection (ATOD) posing significant challenges due to variations in object sizes and backgrounds \cite{ding2021object}. To address these challenges, GANs have been explored \cite{devaguptapu2019borrow, sikdar2024ssl} for IR generation to reduce manual annotation and enhance object detection performance. Recent studies \cite{song2024misaligned, ma2024hierarchical} have explored object detection with misaligned RGB-IR images, revealing the limitations of co-registered datasets. These works emphasize the necessity of advanced techniques such as domain adaptation to address this challenge effectively. \\
% Despite the advancements in RGB cameras, they suffer a major set-back during uncertain environmental conditions such as low-illumination, fog, rain, etc. Due to which a lot of critical applications in context of surveillance and military missions use thermal camera along with RGB to tackle such cases \textbf{cite aniruddhs work}. These works mainly involve sensor fusion on the image space \textbf{cite sensor fusion algos} which require both RGB and thermal images to be co-registered, and they do not account for the pixel shifts that occur during registration process. For which recently D3T \cite{do2024d3t} has proposed domain adaptation technique to handle RGB and IR modalities simultaneously. This work follows the traditional mean-teacher architecture that was originally proposed for Unsupervised Domain adaptation \textbf{Cite mean-teacher work}. Several algorithms such as \cite{cao2023contrastive}, 
\textbf{Domain Adaptive Thermal Object Detection}
% Basics and what is it doing now? \\
% How and why is this important for un-coregistered images?\\
% Domain adaptation for drone imagery - give us 1-2 models, and say its in a nascent stage.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% UDA for object detection focuses mainly about the domain shifts that is seen between two domains i.e. labeled source and unlabeled target domain. UDA methods can be classifed mainly into two categories i.e. domain alignment and self-training. The motivation of domain alignment methods is to reduce the domain discrepancy through feature alignment strategy or using style alignments between the source and target domains this include adversarial training and style transfer techniques. However these approaches are not practically feasible due to establishing the balance between discriminability and feature transferability. And in self-training approaches makes use of the target domain knowledge to achieve superior performance in source domain without labels.  Works such as \cite{deng2021unbiased}, \cite{li2022cross} and \cite{cao2023contrastive} uses mean-teacher architecture to predict pseudo-labels for the target domain using teacher network to guide the student networks performance on target domain. While \cite{cao2023contrastive} implements contrastive learning to achieve self-training. Recently \cite{do2024d3t} proposed two teachers and single student architecture along with zig-zag learning to avoid domain confusion among the teacher network, however the zig-zag learning fails in senarios where the dataset is complex leading to model collapse. This is mainly due to the loss value that increases whenever the learning changes from one teacher to another very immediately which leads to loss tending towards to nan or infinity. Hence our proposed augmentation with all the adaptation algorithms have shown consistent improvement on three dataset including our proposed IndraEye dataset.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
UDA for RGB-to-IR adaptation reduces domain gaps between a labeled source and an unlabeled target. It minimizes discrepancies by aligning features or styles, and self-training. Methods like adversarial training \cite{chen2018domain, hsu2020every} and style transfer \cite{chen2020harmonizing, inoue2018cross, kim2019diversify} aim to bridge domain gaps, but they struggle to balance feature discriminability. Self-training methods enhance performance on the target domain by utilizing source domain knowledge without relying on labels. For example, studies like \cite{deng2021unbiased}, \cite{li2022cross}, and \cite{cao2023contrastive} employ a mean-teacher framework, where a teacher network generates pseudo-labels to guide the student network in the target domain. Recently, \cite{do2024d3t} proposed a two-teacher, single-student architecture with zig-zag learning to reduce domain confusion. However, frequent teacher switching causes loss values to diverge, leading to model collapse on complex datasets. In contrast, our proposed SAGA augmentation, integrated with different adaptation algorithms, consistently enhances performance across multiple datasets. \\
\textbf{Multi-modal Object Detection dataset}
% The usage of RGB-IR images for object detection started initially, with the release of VEDAI dataset that had 12,000 images with 9 categories using drone in the year 2015 which were mostly birds-eye viewed. The need for RGB-IR dataset in autonomous driving was further increased after the release of KAIST dataset for pedestrain detection in the year 2015. Few of these datasets contains images that are misaligned due to poor camera calibration and mechanical vibrations that includes  CVC and KAIST though KAIST was co-registerd using special mechanism of beam splitter. Subsequently a significant increase in such dataset was observed including FLIR (2019), LLVIP (2021), DroneVehicle (2021) and M3FD (2022). Drone based object detection faces lot of challenges due to scale variations and occlusion issues. To tackle this a series of drone based industrial datasets were released including VEDAI and DroneVehicle. LLVIP dataset was captured using video surveillance camera mainly accounting for low light conditions during night time and contains only person class. M3FD dataset was released mainly for fusion approaches which has diverse scenes with high resolution images supporting advanced vision tasks such as detection and segmentation. Conspicuously LLVIP, DroneVehicle and M3FD datasets are collected by manually co-registering the RGB-IR images. Meanwhile since the operation of drone applications are in real-time, manually aligning the image pairs can be both human resource and time consuming. Although alignment accuracy can be achieved using special hardware such as calibration devices and sensors, the algorithms performance is limited due to several factors such as mechanical vibrations, temperature variations, and accuracy of feature matching algorithms, etc. Hence, we constructed a diverse multi-modal misaligned aerial object detection dataset with large classes that highly co-relates with the real-world challenges such as long-tail, scale variations, occlusion.
Datasets like VEDAI \cite{razakarivony2016vehicle} introduced RGB-IR imagery for object detection, featuring 12,000 bird’s-eye-view drone images across nine categories. The KAIST dataset \cite{hwang2015multispectral}, released the same year, focused on pedestrian detection for autonomous vehicles and gained significant traction despite challenges like misalignment caused by mechanical vibrations and calibration errors. While KAIST employed beam-splitter co-registration for alignment, other datasets like CVC14 \cite{gonzalez2016pedestrian} faced persistent alignment issues due to hardware limitations. In subsequent years, more extensive datasets have emerged, including FLIR \cite{fliresh}, LLVIP \cite{jia2021llvip}, DroneVehicle \cite{sun2020drone}, and M3FD \cite{liu2022target}. Drone-based detection presents distinct challenges, such as object occlusion and scale variations, which datasets like VEDAI and DroneVehicle aim to address.
The LLVIP dataset focuses on low-light surveillance for pedestrian detection, while M3FD facilitates multimodal fusion for detection using high-resolution imagery. However, LLVIP, DroneVehicle, and M3FD depend on manual RGB-IR image co-registration, a labor-intensive process unsuitable for real-time drone operations\cite{song2024misaligned}. Hardware-based alignment methods, such as calibration devices or sensors, often struggle due to environmental factors like temperature fluctuations, mechanical instability, and limitations in feature-matching algorithms\cite{brenner2023rgb}. 
Additionally, these datasets contain fewer samples, limited classes, multi-scale variations, and diverse slant angles.
To tackle these challenges, we present the IndraEye dataset, specifically designed to accommodate real-world constraints like long-tail distributions, occlusion, and scale diversity. A qualitative comparison with existing datasets is presented in Table \ref{Qual_comp}. \\
% Labeling multi-modal datasets for object detection is a know problem in the research community. As an alternative unsupervised domain adaptation is introduced to tackle both annotation and domain shifts for any given dataset.


% \subsection{Datasets for RGB-T for drone imagery}
% our dataset not only provides diverse sensing data,

% In addition, we provide a DELIVER benchmark to foster multimodal learning.
% \begin{table*}[h]
% \centering
% \fontsize{7pt}{7pt}\selectfont
% \begin{tabular}{l c c c c c c c}
% \toprule
% \textbf{Datasets} & \multicolumn{1}{l}{\textbf{Multi-sensory}} & \multicolumn{1}{l}{\textbf{Diverse Viewpoints}} & \multicolumn{1}{l}{\textbf{Diverse backgrounds}} & \multicolumn{1}{l}{\textbf{Diverse classes}} & \multicolumn{1}{l}{\textbf{Diverse illumination}} & \multicolumn{1}{l}{\textbf{Detection}} & \multicolumn{1}{l}{\textbf{Segmentation}}\\
% \midrule
% DOTA \cite{xia2018dota}             & \ding{55}                                          & \ding{55}                                                & \ding{55}                                                 & \checkmark                                             & \ding{55}                                    & \checkmark                 & \ding{55}          \\
% HIT-UAV \cite{suo2023hit}         & \ding{55}                                           & \checkmark                                                & \checkmark                                                 & \ding{55}                                             & \ding{55}                             & \checkmark                   & \ding{55}               \\
% VisDrone \cite{cao2021visdrone}        & \ding{55}                                           & \checkmark                                                & \checkmark                                                 & \checkmark                                             & \checkmark                        & \checkmark                   & \ding{55}                                       \\
% UAVDT  \cite{du2018unmanned}           & \ding{55}                                           & \checkmark                                                & \checkmark                                                 & \checkmark                                             & \checkmark                        & \checkmark                   & \ding{55}                                       \\
% Vedai \cite{razakarivony2016vehicle}            & \checkmark                                           & \ding{55}                                                & \checkmark                                                 & \checkmark                                             & \checkmark               & \checkmark                   & \ding{55}                                                \\
% M3FD \cite{liu2022target}             & \checkmark                                           & \ding{55}                                                & \checkmark                                                 & \checkmark                                             & \checkmark                        & \checkmark                   & \ding{55}                                       \\
% FLIR \cite{fliresh}            & \checkmark                                           & \ding{55}                                                & \checkmark                                                 & \checkmark                                             & \checkmark                               & \checkmark                   & \ding{55}                                \\
% MSRS \cite{tang2022piafusion}          & \checkmark                                           & \ding{55}                                              & \checkmark                                                 & \checkmark                                             & \checkmark                                & \ding{55}                   & \checkmark                               \\
% InfraParis \cite{franchi2024infraparis}  & \checkmark                                           & \ding{55}                                              & \checkmark                                                 & \checkmark                                             & \checkmark                                & \checkmark                   & \checkmark                               \\
% {\textbf{IndraEye (Ours)}}   & \checkmark                                           & \checkmark                                                & \checkmark                                                 & \checkmark                                             & \checkmark                                & \checkmark                   & \checkmark                               \\
% \bottomrule
% \end{tabular}

% \caption{Qualitative comparison of multiple aerial vehicle object detection datasets.} 
% \label{table:Dataset comparison}

% \end{table*}








%-------------------------------------------------------------------------
% \subsection{References}

% List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
% When referenced in the text, enclose the citation number in square brackets, for
% example~\cite{Authors14}.
% Where appropriate, include page numbers and the name(s) of editors of referenced books.
% When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
% If you use the template as advised, this will be taken care of automatically.

% \begin{table}
%   \centering
%   \begin{tabular}{@{}lc@{}}
%     \toprule
%     Method & Frobnability \\
%     \midrule
%     Theirs & Frumpy \\
%     Yours & Frobbly \\
%     Ours & Makes one's heart Frob\\
%     \bottomrule
%   \end{tabular}
%   \caption{Results.   Ours is better.}
%   \label{tab:example}
% \end{table}

% %-------------------------------------------------------------------------
% \subsection{Illustrations, graphs, and photographs}

% All graphics should be centered.
% In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
% Instead use
% {\small\begin{verbatim}
%   \centering
% \end{verbatim}}
% at the beginning of your figure.
% Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
% Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
% Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
% You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

% When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
% {\small\begin{verbatim}
%    \usepackage{graphicx} ...
%    \includegraphics[width=0.8\linewidth]
%                    {myfile.pdf}
% \end{verbatim}
% }


% %-------------------------------------------------------------------------
% \subsection{Color}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

% If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
% Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/4_methodology.tex <==
% \section{Methodology}
% \usepackage{graphicx}



\section{Semantic Aware Gray color Augmentation (SAGA) for Domain Adaptation}
% The proposed Semantic Aware Gray color Augmentation (SAGA) and IndraEye dataset are introduced in the following sections. 
% Section 3.1 describes the Mean Teacher framework for unsupervised domain adaptation, adapted for domain-adaptive thermal object detection. Section 3.2 presents the SAGA augmentation method, followed by Section 3.3, which introduces the IndraEye dataset.
The following sections outline SAGA and IndraEye. Section 3.1 outlines the Mean Teacher framework for thermal object detection, Section 3.2 presents SAGA, and Section 3.3 introduces IndraEye.

\subsection{Preliminaries on the Mean Teacher Framework for Domain Adaptation }
% \subsection{Object Detection}
The Mean Teacher (MT) framework \cite{tarvainen2017mean} for domain-adaptive object detection leverages a teacher-student mutual learning framework to transfer knowledge from a labeled source domain to an unlabeled target domain \cite{deng2021unbiased, deng2023harmonious, liu2021unbiased}. Specifically, in the context of domain-adaptive thermal object detection, the source domain comprises RGB images, while the target domain consists of infrared (IR) images.
The teacher and student models are two object detection networks with identical architectures. This framework processes source and target data simultaneously, enabling mutual knowledge transfer. The teacher model, trained on the labeled source domain, generates pseudo labels for the unlabeled target domain data. The student model learns from these pseudo labels, and its updated weights are periodically transferred to the teacher model, enabling continuous improvement. The framework is optimized using the following loss function:
\begin{equation}
    \textit{L} = \textit{L}_{src} + \textit{L}_{tgt}
\end{equation}
where, $L_{src}$ denotes the loss associated with the source domain, while $L_{trt}$  represents the loss for the target domain. The teacher model's weights are updated using the student model's weights through the Exponential Moving Average (EMA) mechanism. Throughout the training process, the teacher model update effectively forms an ensemble of the student model's weights, represented as:
\begin{equation}
    \theta^{T} =  \alpha \theta^{T} + (1-\alpha)\theta^{S}
\end{equation}
where, $ \theta^{T}$   represents the teacher model's weights, while 
$ \theta^{S}$   denotes the student model's weights. CMT \cite{cao2023contrastive} introduces a framework that integrates contrastive learning with the MT methodology, where the student network is trained using stronger augmentations, while the teacher model is trained with weaker augmentations. D3T \cite{do2024d3t}, on the other hand, employs two separate teacher models followed by a zigzag training mechanism. For additional information, please refer to \cite{cao2023contrastive,do2024d3t}.




\subsection{Semantic Aware Gray color Augmentation (SAGA) for Domain Adaptation}
 
Color and structure serve as fundamental elements of an image, both essential for object detection models, with the impact of color bias extensively studied through an emphasis on structural features \cite{hou2020learning, gong2024exploring}. Models trained on RGB data often heavily depend on these color cues, as chromatic diversity is crucial for distinguishing objects in RGB imagery \cite{zhang2022fmcnet}. However, infrared (IR) imaging modalities inherently lack the ability to capture rich color and structural details compared to RGB, posing significant challenges for cross-modal analysis and domain adaptation \cite{zhao2021joint, cheng2023multi}. In the target IR domain, the absence of chromatic diversity leads to a significant reduction in color information, which can contribute to an increased rate of false positives. Domain-adaptive thermal object detection strives to balance the dependence on RGB color bias while retaining essential structural features, in the target IR domain \cite{wu2017rgb}. To mitigate this bias while preserving essential visual cues, we introduce Semantic-Aware Gray Color Augmentation (SAGA), a simple, effective augmentation easily integrated into any object detection algorithm.


When training an object detection model on the source domain using RGB images, let the dataset be represented as \textit{S}=\{$x_i$, $y_i$\}, where $x_{i}$ denotes the images and $y_{i}$  represents the corresponding object labels. These labels are utilized to selectively convert object instances in $x_{i}$ to grayscale while preserving the original color information in the background, rather than applying grayscale conversion to the entire image. SAGA selectively converts object instances to grayscale while retaining the background's color information, ensuring semantic awareness.

Consider an image \textit{I} containing \textit{n} objects, represented as \textit{I} = \{$o_1$, $o_2$, ..., $o_n$\}, where $o_1$, $o_2$, and $o_n$ denote the individual objects within the image. Each object is extracted, converted to grayscale, and then reintegrated into the original image, ensuring that only the object instances appear in grayscale while the background retains its original colors. This process produces a hybrid RGB-grayscale image, as illustrated in Fig. \ref{fig:sagav1}, while preserving the structural integrity of the objects. SAGA can be represented as the following equation, which converts given image \textit{I} by multiplying the red, green and blue channel of each pixels by the values [0.2989, 0.587, 0.114] respectively,
\begin{equation}
    I =  I \times [0.2989, 0.5870, 0.1140]
\end{equation}
RGB-to-IR adaptation highlights that directly transferring knowledge from the RGB source domain to the IR target domain can lead to the transfer of irrelevant features via the EMA technique \cite{do2024d3t}, as there is no explicit mechanism to selectively extract meaningful information. This challenge contributes to an increase in false positives within the pseudo labels generated by the teacher network. To mitigate this, SAGA is integrated into the mean-teacher framework, enabling effective knowledge transfer from labeled RGB images to the unlabeled IR target domain. SAGA is used for domain-adaptive thermal object detection, where source images undergo instance-level gray augmentation to enhance feature adaptation before being trained within their respective frameworks, as shown in Fig. \ref{fig:cmt_saga}.
%The source domain is represented as S = $\{sx_i, sy_i\}_j^N$ where $sx_i$ represents the images, $sy_i$ represent $i^{th}$ the bounding box annotations of the $j^{th}$ image and N represent the total number of images. And target domain is represented by T = $\{tx\}_i^N$ where $tx_i$ represent the $i^{th}$ target image that does not contain any labels. \\
%The proposed augmentation technique is effective in unsupervised domain adaptation thereby enhancing the knowledge transfer from labeled source domain to unlabeled target domain. 
%Particularly we validate the augmentation for RGB-IR domain adaptation since it is known that there is no semantic color information present in the IR domain while it is abundant in RGB images. 
%\begin{equation}
%    \theta^{T} =  \alpha \theta^{T} + (1-\alpha)\theta^{S}
%\end{equation}

%Here $\theta$ represents the parameters of the respective models such as $\theta^T$ for target domain and $\theta^S$ for the source domain.
% \begin{figure}[]
%     \centering
%     \includegraphics[scale=0.43]{images/SAGAV3.png}
%     % \includegraphics[scale=0.2]{images/cmt.png}
%     \setlength{\abovecaptionskip}{-11pt} 
%     \setlength{\belowcaptionskip}{-15pt}
%     \caption{Illustration of SAGA augmentation. The process involves extracting objects from the image, converting them to grayscale, and reintegrating them into the original image while preserving background color information.}
%     \label{fig:sagav1}
% \end{figure}

% \begin{figure}[]
%     \centering
%     \includegraphics[scale=0.43]{images/SAGAV4.png}
%     % \includegraphics[scale=0.2]{images/cmt.png}
%     \setlength{\abovecaptionskip}{-11pt} 
%     \setlength{\belowcaptionskip}{-15pt}
%     \caption{Illustration of SAGA augmentation. The process involves extracting objects from the image, converting them to grayscale, and reintegrating them into the original image while preserving background color information.}
%     \label{fig:sagav1}
% \end{figure}
% \vspace{-4em}
\begin{figure}[]
    \centering
    \includegraphics[scale=0.415]{images/SAGAV5.png}
    % \includegraphics[scale=0.2]{images/cmt.png}
    \setlength{\abovecaptionskip}{-11pt} 
    \setlength{\belowcaptionskip}{-15pt}
    \caption{Illustration of SAGA augmentation. The process involves extracting objects from the image, converting them to grayscale, and reintegrating them into the original image while preserving background color information.}
    \label{fig:sagav1}
\end{figure}


\begin{table}[ht]
\centering

\begin{tabular}{c c c l}
\toprule
\multicolumn{1}{l}{\textbf{Sensor}} & \multicolumn{1}{l}{\textbf{Resolution}} & \multicolumn{1}{l}{\textbf{Wavelength}} & \textbf{FoV} \\ 
\midrule
RGB camera                        & 1280x720                                 & 400-700\text{nm}                                & 60$^\circ$                      \\ 
IR Camera                        & 640x480                                  & 8-14$\mu$m                                     &  32$^\circ$                      \\ 
\bottomrule
\end{tabular}
\caption{Sensor specifications of the DragonEye 2 RGB-IR camera used for the IndraEye dataset.}
\label{sensor_specs}
\end{table}

% To create the IndraEye dataset, we used the DJI M600 Pro drone (Fig. 1), equipped with a DragonEye2 camera mounted on a gimbal to capture various slant-angle views by adjusting pitch and yaw. For low-altitude captures, the camera and gimbal setup were placed on a 3-meter elevated tripod. The DragonEye2 camera includes one Electro-Optical (EO) sensor and one uncooled Infrared (IR) sensor, with detailed specifications provided in Table 2. IndraEye was collected at different times of day—noon, evening, and night—to account for variations in illumination and backgrounds, thereby reducing inherent biases in neural networks (additional examples are available in the supplementary material). After image collection, the dataset was constructed by manually annotating target objects with bounding boxes in both EO and IR data.

% Videos from the EO-IR camera were recorded at seven locations in Bengaluru, including the Indian Institute of Science campus. 
% Dataset at each location was collected for approximately 4 minutes, resulting in about 20,000 frames per scene. To improve object diversity and manage redundant content, every 35th frame was selected for inclusion in the dataset. 
\subsection{Aerial Multi-Modal Perception Dataset}
\textbf{Acquisition process} The IndraEye dataset was collected using a DJI M600 Pro drone equipped with a multi-sensor RGB-IR camera mounted on a gimbal, allowing for image capture from various slant angles by dynamically adjusting the pitch and yaw. The dataset also consists of data collected by mounting the RGB-IR camera on a 3 meter elevated tripod placed over places such as bridge and underpass, there by accounting for low range slant angle that is similar to that of a traffic pole mounted camera images. The information about the sensor can be found in Table \ref{sensor_specs}. IndraEye is one of the very few mutlispatial and multitemporal slant angle dataset available at two modalities i.e. RGB and IR. The dataset was manually structured by annotating the potential objects of interest with bounding boxes in RGB and IR images. The video was shot for approximately 4 to 5 minutes in each of the different locations as shown in Table \ref{table: dataset description_class}. This generated around 20,000 frames per scene as the refresh rate of the RGB camera is 50Hz and that of IR is 10Hz. To avoid redundancy of objects we consider only 35th frame in the video to obtain diverse object rich frames. \\
\textbf{Camera calibration} Recent work \cite{brenner2023rgb} has shown that calibrating RGB and IR camera on a drone vehicle under motion is challenging and not feasible due to the variations in camera parameters such as focal length, field of view (FOV) and refresh rate during movement of the drone. This is a serious issue since most of the camera calibration methods requires computing homography matrix and running feature matching algorithm such as SIFT\cite{lowe2004distinctive}, SURF\cite{bay2006surf} on the device to align both RGB and IR images. This process limits edge-based machine learning due to computational constraints \cite{brenner2023rgb}. Stereo camera calibration is effective but challenged by differing RGB-IR FOVs, leading to depth-dependent parallax \cite{gao2021stereo}. This occurs due to variations in sensor parameters and viewing angles, causing objects at different depths to appear in different image positions. \\
% Due to the hardware and software limitations of the camera, calibrating a system like DragonEye2 where both EO and IR cameras are integrated into a single module mounted on a drone has proven to be challenging \cite{ADD_CITATION}. The difficulty is mainly due to the variations in the camera parameters such as focal length and field of view during the movement of the drone vehicle.
% (because of the variations caused by the focal length of the sensor for better clarity on the object features) the field of view (FoV) varies dynamically with the movement of the drone along with the camera,
% This causes complications in the calibration of the EO and IR sensors as reported by \cite{THE_REVIEW_PAPER}.
% complicating the calibration of both cameras as mentioned in \cite{brenner2023rgb}. 
%While stereo camera calibration is effective, it encounters a significant challenge due to different FOV's of the modalities (RGB-IR) which can result in a parallax effect that varies at different depths \cite{gao2021stereo}. This phenomenon is because of the difference variation in sensor parameters and viewing angles between the cameras, causing objects at various depths to appear at different positions in the image. 
% Consequently, employing a single homography matrix, a transformation that maps points from one image to corresponding points in another is not very effective due to the variation in perspective. 
This misalignment becomes evident in the fused data when the vehicle with the camera is in motion \cite{brenner2023rgb}. Image alignment can lead to inaccuracies, particularly with long distance and small objects. As a result, the process of co-registration is avoided intentionally. While the RGB and IR images are captured with the same timestamp, they still exhibit minor misalignment due to change in refresh rate of the sensor. This limitation highlights the importance of multimodal approaches that eliminate the necessity for co-registered images, such as domain adaptation \cite{do2024d3t}, \cite{gan2023unsupervised}.\\
\textbf{Statistics of the dataset} 
IndraEye comprises 5,612 images that includes multiple viewing angles, altitudes, backgrounds, and times of day. The RGB images are divided into 2,336 samples (2,026 for training, 60 for validation, and 250 for testing), while the IR images are divided into 3,276 samples (2,973 for training, 58 for validation, and 245 for testing). The dataset additionally includes day and night splits. The goal was to create a diverse and comprehensive dataset with both RGB and IR images, suitable for various conditions and contexts.
IndraEye features 13 classes: backhoe loader, bicycle, bus, car, cargo truck, cargo trike (a medium-sized three-wheeled cargo vehicle), ignore, motorcycle, person, rickshaw (a small three-wheeled passenger vehicle), small truck, truck, tractor, and van. More information regarding the dataset is provided in 
% Detailed class distribution for the IndraEye training set is shown in
Table \ref{table: dataset description_class}. To improve object diversity and reduce redundancy, every 35th frame was extracted from the 20,000 frames captured per scene.\\

\textbf{Annotation}  For the IndraEye dataset, we provide ground-truth labels for both object detection and pixel-level semantic segmentation across all classes using a two-stage approach. 
\begin{enumerate}
  \item  \textbf{Zero-Shot Annotations with Human in the Loop:}
    In this initial step, we generate zero-shot annotations by utilizing pre-trained models. These models are used to produce preliminary annotations with human oversight, ensuring that the annotations align closely with the true object locations and characteristics.
    \item \textbf{Manual Verification and Refinement:}
    After generating the initial annotations, each label undergoes thorough manual verification. This step involves a detailed review of the annotations to correct any discrepancies and refine the labels for higher accuracy.
\end{enumerate}

This structured approach ensures that both object detection and pixel-level annotations are meticulously crafted and reliable. For the object detection task, RGB and IR images are manually annotated with bounding boxes using the X-AnyLabeling tool \cite{X-AnyLabeling}. This tool facilitates efficient annotation by allowing users to load pre-trained models, such as those from the YOLO family of networks. After multiple iterations of correction and evaluation, highly precise annotations have been generated.  For semantic segmentation, we use SAMRS \cite{wang2024samrs}, an extension of SAM \cite{kirillov2023segment}, optimized for aerial imagery. SAMRS leverages remote sensing datasets to efficiently generate masks for large-scale segmentation tasks. 
This approach has streamlined our process for producing pixel-level annotations for IndraEye. The annotations for both tasks are carefully designed to match the established class schema.\\
\textbf{Ethics and policy} The proposed dataset undergoes a thorough manual review to ensure privacy protection. Faces of individuals and vehicle license plates that are clearly visible in the images are blurred to maintain confidentiality and safeguard personal rights. This process ensures that individuals' privacy is upheld while preserving the dataset's utility.
\begin{figure}[]
    \centering
    \includegraphics[scale=0.155]{images/cmt_new.png}
    \setlength{\abovecaptionskip}{-5pt} 
    \setlength{\belowcaptionskip}{-11pt}
    \caption{Domain-adaptive thermal object detection with RGB as the source domain and IR as the target domain. (a) Vanilla CMT on the IndraEye dataset. (b) CMT with SAGA on the IndraEye dataset.}
    \label{fig:cmt_saga}
\end{figure}
% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.155]{images/cmtv2.png}
%     \caption{(a) Vanilla CMT on IndraEye dataset and (b) CMT with SAGA on IndraEye dataset}
%     \label{fig:inra}
% \end{figure}




% \section{Augmentation Technique - REMOVE}
% % \subsection{Object Detection}
% We propose an simple and efficient augmentation strategy that can be used with any object detection algorithm. This is validated on two different use cases as illustrated below:
% \newline\textbf{1. Augmentation on Object Detection tasks:} \\
%  Color and structure considered as the two main pillars of an image that is used in CNN's for various tasks and the effect of color bias in CNNs is addressed in \cite{hou2020learning} by focusing on only the structure. \cite{gong2024exploring} work tries to mitigate the color bias problem but is not explored for object detection and performs experiments only for person re-identification and uses ensemble technique to achieve superior performance. In this work, we propose a novel augmentation strategy is used on RGB images to mitigate the color bias issue in CNNs. Consider a batch of object detection dataset denoted as S = \{$x_i$, $y_i$\}, where $x_i$ denotes the batch of images and yi represents the batch of corresponding object labels for the respective images. We make use of the object labels to convert the object instances to grey color and retain the color information of the background. We perform extensive analysis and conclude that converting the entire image to grey color does not yield better performance in comparison to our proposed grey scale augmentation.
% \vspace{0.5em}
% \textbf{\hrule}
% \vspace*{0.4em}
% \hspace{-1em}\textbf{Algorithm} Instance level grey scale augmentation \vspace{0.4em}
% \textbf{\hrule}
% \vspace*{0.4em}
% \hspace{-1em}\textbf{Input}: S = \{$x_i$, $y_i$\}, $x_i$ and $y_i$ represents the image and annotation labels respectively.
% \newline 1: \textbf{for} image in S:
% \newline 2: \quad Initialize temp
% \newline 3: \quad Initialize grey $\leftarrow$ [0.2989, 0.5870, 0.1140]
% \newline 4: \qquad \textbf{for} annotations in $y_i$:
% \newline 5: \qquad xmin, ymin, xmax, ymax $\leftarrow$ annotations["bbox"]
% \newline 6: \qquad croppedimg $\leftarrow$ image[ymin:ymax, xmin:xmax]
% \newline 7: \qquad instgry $\leftarrow$ croppedimg @ grey
% \newline 8: \qquad \textbf{end for}
% \newline 9: \quad temp = image[$y_i$]
% \newline 10: \quad temp = temp @ grey
% \newline 11: \quad image[ymin:ymax, xmin:xmax] $\leftarrow$ temp
% \newline 12: \qquad \textbf{end for}
% % \newline 13: \quad return image
% \newline \textbf{Output:} Instance level grey image with label $y_i$ \\

% \hspace{-1em}This can be represented as the following equation which is rendered from the pytorch function \verb|rgb_to_grayscale| which converts any given image by multiplying the red, green and blue channel of each pixels by the values [0.2989, 0.587, 0.114] respectively.

% \centerline{$X$ = $X$ $\times$ [0.2989, 0.5870, 0.1140]}

% \hspace{-1em}Consider and image I with ``n'' objects represented as I = \{$o_1$, $o_2$, ..., $o_n$\} where $o_1$, $o_2$, and $o_n$ are objects in the given image, we extract the objects from the image and convert them to grey color image and them append the object patches back to the original image which has the object alone converted to grey color. This generates the image as shown in Fig. . This process generates a combination of RGB and grey image while preserving the structural integrity of the objects.
% \subsection{Unsupervised Domain Adaptation}


% Unsupervised domain adaptation is used to mitigate the domain gap between two domains in which one domain has labels and the other domain has no labels while training. This method usually includes a student and a teacher model. Traditionally the teacher network uses only the target data and does not perform back-propagation and the weights are updated from the student network through EMA technique. The student network learns from both source and target domain and is finally used during evaluation.  
% We evaluate our methodology on Unsupervised domain adaptation to verify the effectiveness of knowledge distillation from RGB to IR modality. We consider the RGB domain as source i.e with labels and IR data as target domain without labels. We verify the results on mean-teacher based architectures.


 

 
% We evaluate our proposed methodology on three different datasets for object detection task including FLIR, LLVIP and our proposed dataset i.e. IndraEye. Notably FLIR dataset is collected in horizontal view for autonomous ground vehicles while IndraEye is collected in slant angle for autonomous aerial vehicle that accounts for the varying scale and occlusion issues seen during slant angle. This study proves that the proposed augmentation strategy is robust to scale and occlusion problems which is commonly seen in real world datasets. 

==> sec/5_experimental.tex <==
\section{Experiments}
In this section, we present the experimental results of the proposed SAGA on state-of-the-art unsupervised domain adaptation models, including D3T \cite{do2024d3t}, CMT \cite{cao2023contrastive}, and AT \cite{li2022cross}. These models are evaluated on two open-source datasets, FLIR \cite{zhang2020multispectral} and LLVIP \cite{jia2021llvip}, along with the proposed IndraEye dataset. We also assess object detection models across various settings to establish a benchmark on the IndraEye dataset.


% \textbf{How is this??}
% In this section, we demonstrate the effectiveness of our proposed augmentation SAGA for Unsupervised RGB-T domain adaptation by comparing with recent state-of-the-art algorithms and datasets. We also demonstrate the importance of aerial RGB-T dataset for object detection mainly for approaches like domain adaptation. We show that SAGA with the state-of-the-art unsupervised domain adaptation technique beats the networks without SAGA by a significant margin as shown in the results.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[scale=0.3]{images/pred.png}
%     \caption{Output predictions to higlight the importance of the SAGA augmentation.}
%     \label{fig:pred}
% \end{figure*}

% Decrease the size of this font
% \subsection{Datasets}
% % \textbf{Dataset and Evaluation Metrics}
% 

% \textbf{How is this??}

\subsection{Datasets and Evaluation metric }
%\textbf{Datasets: } We perform all the experiments for SAGA on three RGB-T datasets two of which are publicly available and are used for object detection task i.e. FLIR-ADAS and LLVIP and thirdly we evaluate all the methods on our dataset to set the benchmark. FLIR-ADAS dataset has 9,214 thermal and RGB image pairs and has mainly three class labels car, person, and bicycle. The dataset contains images of resolution 640 x 512 and are collected during both day and night images. All experiments are carried out on the official training and testing split provided. To demonstrate the effect of lighting condition, LLVIP dataset is chosen and consists of only night-time images. It has 15,488 RGB-T image pairs and each image has a resolution of 1080x720 pixels and LLVIP has only person class. IndraEye dataset consists of 5,612 RGB and 3276 thermal images collected during all times of the day and night. And notably it has 13 vehicle objects i.e. car, backhoe loader, bus, van, bicycle, cargo truck, ignore, cargo trike, small truck, motorcycle, person, tractor, truck and rickshaw. \\
\textbf{Datasets}  Experimental evaluation is conducted using the FLIR, LLVIP, and IndraEye datasets. FLIR \cite{zhang2020multispectral} is collected from an autonomous driving perspective. This dataset consists of 5,142 aligned RGB-IR image pairs, with 4,129 images allocated for training and 1,013 for testing, covering daytime and nighttime scenes. LLVIP \cite{jia2021llvip} is a low-light vision dataset captured from a slant angle, roughly three stories above ground. It contains 15,488 RGB-IR image pairs, mainly featuring extremely dark scenes and focusing solely on the Pedestrian class.
IndraEye is a slant-angle dataset with 2,336 RGB and 3,276 IR images. Captured from diverse backgrounds and angles, it covers 13 classes, including vehicles and pedestrians, with day and night scenes under varying illumination.\\
\textbf{Evaluation metrics} For experimental validation, we evaluate all the networks using the Mean Average Precision (mAP) score, calculated from precision and recall scores. An mAP threshold of 0.5 is used for all experiments. \\
% \begin{table}[]
% \centering
% \fontsize{9pt}{9pt}\selectfont
% \begin{tabular}{|c|c c c|}
% % \toprule
% \hline
% Algorithm\textbackslash{}Dataset & FLIR & LLVIP & IndraEye \\
% % \midrule
% \hline
% D3T                              & 61.8 & 88.1  & 30.3     \\
% % \midrule
% \hline
% D3T*                             & \textbf{66.1} & \textbf{88.5}  & \textbf{32.9}     \\
% % \midrule
% \hline
% CMT                              & 63.3 & 41.6  & 17.1     \\
% % \midrule
% \hline
% CMT*                             & \textbf{65.7} & \textbf{49.2}  & \textbf{19.3}     \\
% % \midrule
% \hline
% AT                               & TR     & TR      &TR          \\
% % \midrule
% \hline
% AT*                              &  TR    &  TR     &  TR        \\
% % \midrule
% \hline
% Source                           &  37.8    &  82.8     & \textbf{50.5}         \\
% % \midrule
% \hline
% Oracle                           & 67.5     &  83     &   \textbf{65.5}       \\
% % \bottomrule
% \hline
% \end{tabular}
% \caption{Performance comparison with state-of-the-art methods on FLIR, KAIST and our proposed dataset \newline * indicates with the propose augmentation strategy on the respective algorithms}
% \label{table:UDA_results}
% \end{table}
%\vspace{0.5em}
%\hspace{-1em}{}
\textbf{Implementation Details} 
For evaluating domain adaptation networks, we train the models using strategies from \cite{do2024d3t}, \cite{cao2023contrastive}, and \cite{li2022cross}. During the burn-up stage, the student network trains on the source domain for 10,000 iterations. Adaptation to the target domain occurs in subsequent iterations, with a total of 50,000 iterations on the FLIR and LLVIP datasets. For the IndraEye dataset, we train all algorithms for 20,000 iterations, as the D3T \cite{do2024d3t} network diverges after this point, leading to poor results. We hypothesize this is due to the dataset's complexity and the frequent alternation between the student and teacher networks during training (zig-zag training). All experiments in \ref{table:UDA_results} used a batch size of 16 on four NVIDIA V100 GPUs with a VGG16 backbone and the same hyperparameters as the respective works. \\
Object detection models, including FasterRCNN, ReDet, and ORCNN, were benchmarked on the IndraEye dataset using four Nvidia V100 GPUs with a batch size of 6.
We employed the SGD optimizer with a learning rate of 0.0025, weight decay of 0.0001, and momentum of 0.9, training for 12 epochs. The YOLOv8\cite{yolov8_ultralytics} model was trained with a learning rate of 0.00001, a batch size of 16, and an image size of 640 for a total of 100 epochs.

% \textbf{Implementation Details} 
% For evaluating domain adaptation networks, we train the models using strategies from \cite{do2024d3t}, \cite{cao2023contrastive}, and \cite{li2022cross}. During burn-up stage, the student network trains on the source domain for 10,000 iterations. Adaptation to the target domain occurs in subsequent iterations until 50,000 iterations on the FLIR and LLVIP datasets. For the IndraEye dataset, we train all algorithms for 20,000 iterations, as the D3T \cite{do2024d3t} network diverges after this point, leading to poor results. We hypothesize this is due to the dataset's complexity and the frequent alternation between the student and teacher networks during training (zig-zag training). All experiments in Table \ref{table:UDA_results} were conducted with a batch size of 16 on four NVIDIA V100 GPUs with a VGG16 backbone and the same hyperparameters as the respective works.
% Object detection models, including FasterRCNN, ReDet, and ORCNN, were benchmarked on the proposed dataset using 4 Nvidia V100 GPUs with a batch size of 6.
% We employed SGD optimizer with a learning rate of 0.0025, weight decay of 0.0001, and momentum of 0.9, training for 12 epochs. The YOLOv8\cite{yolov8_ultralytics} model was trained with a learning rate of 0.00001, a batch size of 16, and an image size of 640 for a total of 100 epochs.
% For object detection, the  model is trained at Yolov8x’s default hyper-parameter settings with epoch set to 100. \textbf{Tell me training strategies for Table 4.}


%\textit{The works by AT \cite{li2022cross} and CMT \cite{cao2023contrastive} have used Detectron2 library \cite{wu2019detectron2}, while D3T \cite{do2024d3t} is coded using cvpods \cite{zhu2020cvpods} library and faster-rcnn is using mmdetection library \cite{mmdetection}.} 



\begin{table}[]
\centering
\resizebox{3.2in}{!}{
\begin{tabular}{@{}c c c c c c@{}}
\toprule
% \rowcolor[HTML]{9B9B9B} 
\textbf{Models} & \textbf{Train on RGB} & \textbf{Test on RGB} & \textbf{Train on IR} & \textbf{Test on IR} & \textbf{mAP50} \\ 
\midrule
FasterRCNN \cite{NIPS2015_14bfa6bb}     & \checkmark                   & \checkmark                  & \ding{55}                   & \ding{55}                  & 47.6 \\ 

ReDet \cite{han2021redet}          & \checkmark                   & \checkmark                  & \ding{55}                   & \ding{55}                  & 43.9 \\ 

ORCNN \cite{xie2021oriented}          & \checkmark                   & \checkmark                  & \ding{55}                   & \ding{55}                  & 56.3 \\ 

Faster RCNN \cite{NIPS2015_14bfa6bb}    & \ding{55}                   & \ding{55}                  & \checkmark                   & \checkmark                  & 57.3 \\ 

ReDet \cite{han2021redet}          & \ding{55}                   & \ding{55}                  & \checkmark                   & \checkmark                  & 43.8 \\ 

ORCNN \cite{xie2021oriented}          & \ding{55}                   & \ding{55}                  & \checkmark                   & \checkmark                  & 65.6 \\ 
\bottomrule
\end{tabular}}
% \label{fig:detection-dota11}
% \caption{Add citations and table legend.}
% \end{table}
\caption{Performance of object detection algorithms on the proposed IndraEye dataset.}
\label{table:obj_det benchmark ie}
\end{table}


\subsection{Experimental Results}

% \centering
% \begin{figure*}[h]
%     \centering
%     \includegraphics[scale=0.31]{images/cmt_pred.png}
%     \caption{Output predictions to highlight the importance of the SAGA augmentation. (a) RGB image and (b) IR image from the dataset. (c) Demonstration of the challenges faced by a state-of-the-art algorithm on the dataset. (d) Significant reduction in false positives (highlighted with red circles in (c) and (d)) achieved through the proposed SAGA augmentation, showcasing its effectiveness}
%     \label{fig:pred}
% \end{figure*}

\subsubsection{Unsupervised Domain Adaptation}
As observed in table \ref{table:UDA_results}, the proposed SAGA consistently enhances the performance of both CMT and D3T across all three datasets. Specifically, it improves CMT by 2.4 mAP on FLIR, 3.6 mAP on LLVIP, and 2.2 mAP on IndraEye respectively. Similarly, it enhances the performance of D3T by 4.29 mAP on FLIR. Similar trends are observed in other settings. This clearly demonstrates that transferring all information from the student to the teacher is not beneficial. Instead, mitigating color bias while preserving semantic information leads to consistently better performance. This makes the proposed augmentation technique highly effective for RGB-IR domain adaptation, as it consistently improves performance across different look angles, which is crucial for drone imagery. \\
\textbf{Compatibility with existing techniques.} Table \ref{table:abalation} demonstrates that SAGA is compatible with various existing techniques along with domain adaptation approaches. For methods designed to enhance the representation capacity of encoders, such as Jigen\cite{carlucci2019domain}, SAGA does not negatively impact training despite being an augmentation technique. Instead, it complements these methods, supporting their learning and improving the representation ability of models for RGB-IR adaptation. \\
\textbf{Comparison with augmentation techniques:}Although grayscale augmentation helps align RGB to Thermal for domain adaptation, we show that full grayscale augmentation reduces CMT model performance on the FLIR dataset, as observed in table \ref{table:abalation_grey}.
Converting the entire image to grayscale removes important local details, like fine boundaries, making it difficult for the model to identify key features. In contrast, instance-level grayscale augmentation retains these details, enhancing performance.\\
\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.35]{images/cmt_pred.png}
    \setlength{\abovecaptionskip}{-1pt}
    \setlength{\belowcaptionskip}{-8pt}
    \caption{Output predictions to highlight the importance of the SAGA augmentation on CMT algorithm. (a) and (c) shows the increase in false positives while using vanilla CMT. Meanwhile (b) and (d) shows the reduction in false positives when using SAGA with CMT, showcasing its effectiveness.}
    \label{fig:pred_1}
\end{figure}
\textbf{Qualitative results}  Qualitative predictions show improved performance for small-scale objects (Fig. \ref{fig:pred_1}), a common challenge in IR imagery. Unlike RGB, IR sensors lose information from certain viewpoints, especially when objects are viewed from different angles. Grayscale augmentation helps address this issue. We observe a significant reduction in false positives in the vanilla CMT model, and incorporating the proposed augmentation effectively mitigates this problem, while consistently improving performance across three benchmarked datasets, as shown in Table \ref{table:UDA_results}.



% \begin{table}[]
% \centering
% \fontsize{9pt}{9pt}\selectfont
% \begin{tabular}{|c|c c c|}
% % \toprule
% \hline
% Algorithm\textbackslash{}Dataset & FLIR & LLVIP & IndraEye \\
% % \midrule
% \hline
% D3T                              & 61.8 & 88.1  & 30.3     \\
% % \midrule
% \hline
% D3T*                             & \textbf{66.1} & \textbf{88.5}  & \textbf{32.9}     \\
% % \midrule
% \hline
% CMT                              & 63.3 & 41.6  & 17.1     \\
% % \midrule
% \hline
% CMT*                             & \textbf{65.7} & \textbf{49.2}  & \textbf{19.3}     \\
% % \midrule
% \hline
% AT                               & TR     & TR      &TR          \\
% % \midrule
% \hline
% AT*                              &  TR    &  TR     &  TR        \\
% % \midrule
% \hline
% Source                           &  37.8    &  82.8     & \textbf{50.5}         \\
% % \midrule
% \hline
% Oracle                           & 67.5     &  83     &   \textbf{65.5}       \\
% % \bottomrule
% \hline
% \end{tabular}
% \caption{Domain adaptation ablation experiments - Jigen and all settings, on .. dataset. - check table and figure legends, is it above or below.}
% \label{table:UDA_results}
% \end{table}



% \begin{table}[]
% % \caption{Table illustrating how the features of the two modalities complement each other, utilizing a day-night split within the train-test split of the IndraEye dataset.}
% \label{EO-D+N}
% \centering
% \fontsize{7pt}{7pt}\selectfont
% \resizebox{3in}{!}{
% \begin{tabular}{l l l l}
% % \rowcolor[HTML]{9B9B9B}
% \toprule
% \textbf{Algorithm} & \textbf{FLIR} &
% \textbf{LLVIP} &
% \textbf{IndraEye} &
% % \textbf{IndraEye} \\
% % \textbf{mAP50} \\ 
% % \vspace{0.5em}
% \midrule
% D3T    & 61.8     & 88.1   & 30.3          \\ 
% \vspace{0.1em}
% \textbf{D3T + proposed}   & \textbf{66.1 (+4.3)}   & \textbf{88.5 (+0.4)}     & \textbf{32.9 (+2.6)}        \\ 
% \vspace{0.1em}
% CMT    & 63.3   & 41.6     & 17.1      \\ 
% \vspace{0.1em}
% \textbf{CMT + proposed}   & \textbf{65.7 (+2.4)}    & \textbf{49.2 (+7.6)}     & \textbf{19.3 (+2.2)}       \\ 
% \vspace{0.1em}
% % AT       & 48.13   & TR     & 30.4       \\ 
% % \vspace{0.1em}
% % AT + proposed      & TR   & 30.0     & 30.4       \\ 
% % \vspace{0.1em}
% \midrule
% Source       & 37.8   & 82.8     & 50.5       \\ 
% \midrule
% % \vspace{0.1em}
% Oracle       & 67.5   & 83     & 65.5       \\ 
% % \vspace{0.1em}

% \bottomrule
% \end{tabular}}
% \caption{Domain adaptation ablation experiments - Jigen and all settings, on .. dataset. - check table and figure legends, is it above or below.}
% \label{table:UDA_results}
% \end{table}




\begin{table}[h]
% \caption{Table illustrating how the features of the two modalities complement each other, utilizing a day-night split within the train-test split of the IndraEye dataset.}
% \label{table:algo}
\centering
% \fontsize{9pt}{9pt}
\begin{tabular}{l l l l}
% \rowcolor[HTML]{9B9B9B}
\toprule
\textbf{Algorithm} & \textbf{FLIR} &   \textbf{LLVIP} &  \textbf{IndraEye} \\
\midrule
% \vspace{-0.2em}
Source       & 37.8   & 82.8     & 50.5       \\ 
% \vspace{-0.2em}
\midrule
% \vspace{-0.2em}
Oracle       & 67.5   & 83     & 65.5       \\ 
% \vspace{-0.2em}
\midrule
D3T    & 61.8     & 88.1   & 30.3          \\ 
% \vspace{0.1em}
D3T + SAGA   & \textbf{66.1}   \textcolor{forestgreen}{$\uparrow4.3$}  &  \textbf{88.5} \textcolor{forestgreen}{$\uparrow0.4$}   & \textbf{32.9}  \textcolor{forestgreen}{$\uparrow2.6$}    \\ 
% \vspace{0.1em}
CMT    & 63.3   & 41.6     & 17.1      \\ 
% \vspace{0.1em}
CMT + SAGA   & \textbf{65.7}  \textcolor{forestgreen}{$\uparrow2.4$}   & \textbf{49.2}   \textcolor{forestgreen}{$\uparrow7.6$}    &  \textbf{19.3}  \textcolor{forestgreen}{$\uparrow2.2$}      \\ 
% \vspace{0.1em}
% AT       & 48.13   & TR     & 30.4       \\ 
% \vspace{0.1em}
% AT + proposed      & TR   & 30.0     & 30.4       \\ 
% \vspace{0.1em}
% \vspace{0.1em}

\bottomrule
\end{tabular}
% \caption{Domain adaptation ablation experiments - Jigen and all settings, on .. dataset. - check table and figure legends, is it above or below.}
\caption{Experimental Results on State-of-the-art algorithms on two standard datasets i.e, FLIR and LLVIP. Source refers to the accuracy obtained by training on RGB domain and testing on IR domain, while Oracle refers to training and testing on the same i.e. IR domain.}
\label{table:UDA_results}
\end{table}
% \begin{table}[h]
% % \caption{Table illustrating how the features of the two modalities complement each other, utilizing a day-night split within the train-test split of the IndraEye dataset.}
% % \label{table:algo}
% \centering
% % \fontsize{9pt}{9pt}
% \begin{tabular}{l l l l}
% % \rowcolor[HTML]{9B9B9B}
% \toprule
% \textbf{Algorithm} & \textbf{FLIR} &   \textbf{LLVIP} &  \textbf{IndraEye} \\
% \midrule
% % \vspace{-0.2em}
% Source       & 37.8   & 82.8     & 50.5       \\ 
% % \vspace{-0.2em}
% \midrule
% % \vspace{-0.2em}
% Oracle       & 67.5   & 83     & 65.5       \\ 
% % \vspace{-0.2em}
% \midrule
% D3T    & 61.8     & 88.1   & 30.3          \\ 
% % \vspace{0.1em}
% D3T + proposed   & 66.1   &88.5     &32.9        \\ 
% % \vspace{0.1em}
% CMT    & 63.3   & 41.6     & 17.1      \\ 
% % \vspace{0.1em}
% CMT + proposed   &65.7    &49.2     &19.3       \\ 
% % \vspace{0.1em}
% % AT       & 48.13   & TR     & 30.4       \\ 
% % \vspace{0.1em}
% % AT + proposed      & TR   & 30.0     & 30.4       \\ 
% % \vspace{0.1em}
% % \vspace{0.1em}

% \bottomrule
% \end{tabular}
% % \caption{Domain adaptation ablation experiments - Jigen and all settings, on .. dataset. - check table and figure legends, is it above or below.}
% \caption{Experimental Results on State-of-the-art algorithms on two standard datasets i.e, FLIR and LLVIP - \textbf{Add ablation table.}}
% \label{table:UDA_results}
% \end{table}


% \begin{table}[h]
% \centering
% \begin{tabular}{@{}l l l l l@{}}
% \toprule
% \textbf{Model}  &  \textbf{Vanilla} & \textbf{Full gray} & \textbf{Inst-gray} &  \textbf{mAP} \\ \midrule
% \multirow{3}{*}{CMT}  &  \checkmark     &       &        & 63.3 \\
%       &    \ding{55}    &   \checkmark      &      & 61.1 \\
%       & \ding{55}     &   \ding{55}  &  \checkmark  & 65.7 \\ \bottomrule
% \end{tabular}
% \caption{Table illustrating the ablation study of SAGA augmentation on CMT network. \textbf{Dataset?}}
% \end{table}

% to showcase the performance of these models when there is a mixture of scale-variability, diverse illumination and background conditions.
\subsubsection{Benchmarking on IndraEye dataset}
{\textbf{Object Detection}}
Detection models like ReDet \cite{han2021redet}, ORCNN \cite{xie2021oriented}, and Faster-RCNN \cite{NIPS2015_14bfa6bb} show limited in-domain performance (training and testing on the same modality), falling short of real-world, safety-critical application requirements, as shown in Table \ref{table:obj_det benchmark ie}. This can be attributed to factors like scale variability, varying illumination and background conditions, and challenges specific to RGB sensors, which are common in drone imagery. This highlights the significance of the IndraEye dataset and the need for model architectures that are generalizable and adaptable to diverse scenarios.  \\
Table \ref{table:detection-aerial} evaluates the performance of Yolov8x \cite{Jocher_Ultralytics_YOLO_2023} on IndraEye on five different configurations. The four configurations include: first, training on the RGB modality with daytime images and testing on nighttime images under low illumination conditions, highlighting the limitations of RGB imagery in low-light environments. The second configuration assesses the effectiveness of using only RGB sensors for aerial perception, where training incorporates both day and nighttime images, but inference is conducted solely under nighttime conditions. The third configuration is completely based on the capability of the model learning from the IR imagery. Precisely, in this setting IR modality with both day and nighttime images are used to train the DNN. As can be seen from the table \ref{table:detection-aerial}, comparison from the first three test configurations, it is clear that the IR modality is better suited for low-illumination conditions. The fourth and fifth configurations are counterparts to the second and third, evaluated under well-illuminated (daytime) conditions. Results show that RGB sensors, capturing rich texture, perform better in these conditions, while IR sensors excel in low-light environments due to their ability to capture thermal emissivity. \\
To benchmark other aerial perception datasets against IndraEye in the RGB domain, we train YOLOv8x on the VisDrone dataset, which has more training image instances than IndraEye. For a fair comparison, we focus on the common classes (5 classes) between both datasets. Despite VisDrone's larger training set, the cross-domain gap (between IndraEye to VisDrone and VisDrone to IndraEye) reveals that the IndraEye dataset helps the model generalize better, as shown in Table \ref{table:visdrone_table}. We attribute this improvement to the greater diversity and higher quality annotations in the IndraEye dataset.

% Table \ref{fig:detection-dota} assesses the performance of state-of-the-art detection models on nadir-view aerial imagery. While these models demonstrate high performance on other datasets, their effectiveness on the IndraEye dataset is relatively limited. Specifically for EO images, the challenges of densely packed objects, varying slant angles, and diverse illumination conditions contribute to the restricted performance on the IndraEye dataset. \\


% \begin{table}[]
% \caption{Table illustrating how the features of the two modalities complement each other, utilizing a day-night split within the train-test split of the IndraEye dataset.}
% \label{EO-D+N}
% \centering
% \fontsize{7pt}{7pt}\selectfont
% \resizebox{3in}{!}{
% \begin{tabular}{l l l}
% % \rowcolor[HTML]{9B9B9B}
% \toprule
% \textbf{\begin{tabular}[c]{@{}c@{}}Train Setting\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Test Configuration\end{tabular}} & \textbf{mAP50} \\ 
% % \vspace{0.5em}
% \midrule
% EO-Day                                                     & EO-Night                                                                  & 30.0            \\ 
% % \vspace{0.5em}
% EO-Day + EO-Night                                                      & EO-Night                                                                  & 52.0            \\ 
% % \vspace{0.5em}
% IR-Day + IR-Night                                                      & IR-Night                                                                  & 73.6           \\ 
% % \vspace{0.5em}
% EO-Day  + EO-Night                                                      & EO-Day                                                                  & 90.7           \\ 
% % \vspace{0.5em}
% IR-Day + IR-Night                                                      & IR-Day                                                                  & 77.0            \\ 
% \bottomrule
% \end{tabular}}
% \label{table:detection-aerial}
% \end{table}


\begin{table}[]
\label{EO-D+N}
\centering
\begin{tabular}{l l l}
% \rowcolor[HTML]{9B9B9B}
\toprule
\textbf{\begin{tabular}[c]{@{}c@{}}Train Setting\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Test Configuration\end{tabular}} & \textbf{mAP50} \\ 
\midrule
RGB-Day   & RGB-Night    & 30.0   \\ 
RGB-Day + RGB-Night  & RGB-Night  & 52.0  \\ 
IR-Day + IR-Night  & IR-Night  & 73.6   \\ 
RGB-Day  + RGB-Night  & RGB-Day   & 90.7    \\ 
IR-Day + IR-Night & IR-Day    & 77.0   \\ 
\bottomrule
\end{tabular}
\caption{Table illustrating the features of the two modalities complementing each other, utilizing a day-night split within the train-test split of the IndraEye dataset.}
\label{table:detection-aerial}
\end{table}


\hspace{-1em}


\begin{table}[h]
\centering
\fontsize{9pt}{9pt}
\label{DG}
% \fontsize{7pt}{7pt}\selectfont
% \scriptsize   # This is to resize the table to smaller dimension
% \resizebox{1.7in}{!}{
% \begin{tabular}{@{}lll@{}}
% \toprule
% \textbf{Train set} & \textbf{Test set} & \textbf{mAP50} \\ 
% \midrule
% VisDrone           & VisDrone \textbf{cite}         & 53.3           \\ 
% IndraEye           & VisDrone          & 32.5           \\ 
% IndraEye           & IndraEye          & 83.135         \\ 
% VisDrone           & IndraEye          & 52.085         \\
% \bottomrule
% \end{tabular}}
\begin{tabular}{lll}
\toprule
\textbf{Train set} & \textbf{Test set} & \textbf{mAP50} \\ 
\midrule
VisDrone           & VisDrone \cite{zhu2021detection}        & 53.3           \\ 
IndraEye           & VisDrone          & 32.5  \hspace{0.5em}  \textcolor{red}{$\downarrow20.8$}        \\ 
IndraEye           & IndraEye          & 83.1         \\ 
VisDrone           & IndraEye          & 52.1    \hspace{0.5em}  \textcolor{red}{$\downarrow31.05$}    \\
\bottomrule
\end{tabular}
\caption{Generalization of object detection model trained on Visdrone RGB imagery datasets.}
\label{table:visdrone_table}
\end{table}


==> sec/6_abalation.tex <==
%\section{Ablation}

% \begin{table}[h]
% \centering
% \begin{tabular}{@{}l l l l l l@{}}
% \toprule
% \textbf{Model}  &  \textbf{Vanilla} & \textbf{Full gray} & \textbf{SAGA} &  \textbf{Jigen} &  \textbf{mAP} \\ \midrule
% \multirow{3}{*}{CMT}  &  \checkmark     &       &      &     & 63.3 \\
%       &    \ding{55}    &   \checkmark      &     &     & 61.1 \\
%       & \ding{55}     &   \ding{55}  &  \checkmark     &     & 65.7 \\ 
%       & \ding{55}   & \ding{55}   & \ding{55}  & \checkmark   & 68.2 \\ \bottomrule
% \end{tabular}
% \caption{Table illustrating the ablation study of SAGA augmentation and Jigen Pretraining effect on CMT architecture}
% \label{table:abalation}
% \end{table}


\begin{table}[h]
\centering
\begin{tabular}{@{}l l l l l l@{}}
\toprule
\textbf{Model}  &  \textbf{Vanilla} & \textbf{Full gray} & \textbf{SAGA} &  \textbf{mAP50} \\ \midrule
\multirow{3}{*}{CMT}  &  \checkmark     &       &     & 63.3 \\
      &    \ding{55}    &   \checkmark      &     & 61.1 \\
      & \ding{55}     &   \ding{55}  &  \checkmark    & 65.7
      % & \ding{55}   & \ding{55}   & \ding{55}  & \checkmark   & 68.2 
      \\ \bottomrule
\end{tabular}
\caption{Table illustrating the ablation study of SAGA augmentation and Jigen Pretraining effect on CMT architecture.}
\label{table:abalation_grey}
\end{table}



\begin{table}[h]
\centering
\begin{tabular}{@{}l l l@{}}
\toprule
\textbf{Model}  &   \textbf{mAP50} \\ \midrule
Oracle      & 63.3 \\
Source  & 61.1 \\  \midrule
D3T  & 61.8 \\
D3T+SAGA  &  66.1 \\
D3T + Jigen  &  61.5  \\  \midrule
D3T + SAGA + Jigen  &  \textbf{68.2} \hspace{0.3em} \textcolor{forestgreen}{$\uparrow6.4$} \\  \midrule
CMT  & 65.7 \\ 
CMT + SAGA  &  65.7  \\
CMT + Jigen  &  64.7  \\ \midrule
CMT + SAGA + Jigen  &  \textbf{68.3} \hspace{0.3em}  \textcolor{forestgreen}{$\uparrow2.6$} \\
\bottomrule
\end{tabular}
\caption{SAGA on state-of-the-art domain adaptation methods, highlighting its compatibility with existing techniques like Jigen.}
\label{table:abalation}
\end{table}

==> sec/7_conclusion.tex <==
\section{Conclusion}
In this paper, we present Semantic-Aware Gray color Augmentation (SAGA), a novel technique that mitigates color bias and bridges the domain gap by extracting relevant object-level features for IR images. By integrating SAGA with the mean-teacher framework, we enable efficient knowledge transfer from labeled RGB images to unlabeled IR domains thereby achieving consistent performance gains of +0.4$\%$ to +7.6$\%$ when integrated with SOTA domain adaptation methods. To tackle the scarcity of RGB-IR drone imagery datasets, we present IndraEye, the first multisensor aerial perception dataset tailored for diverse classes and illumination conditions. The dataset includes diverse background environments and scene characteristics, featuring 2,336 RGB images and 3,276 IR images across different viewing angles, altitudes, and times of day. Our experimental results demonstrate that SAGA significantly enhances RGB-to-IR adaptation for autonomous driving and the IndraEye dataset. 

\section{Acknowledgments}
This work was supported by The Bengaluru Traffic Police (BTP), The Ministry of Electronics and Information Technology (MeitY) \& The Kotak IISc AI–ML Centre (KIAC).
